Beyond Pixels: Visual Metaphor Transfer via Schema-Driven Agentic Reasoning

A visual metaphor constitutes a high-order form of human creativity, employing cross-domain semantic fusion to transform abstract concepts into impactful visual rhetoric. Despite the remarkable progress of generative AI, existing models remain largely confined to pixel-level instruction alignment and surface-level appearance preservation, failing to capture the underlying abstract logic necessary for genuine metaphorical generation. To bridge this gap, we introduce the task of Visual Metaphor Transfer (VMT), which challenges models to autonomously decouple the "creative essence" from a reference image and re-materialize that abstract logic onto a user-specified target subject. We propose a cognitive-inspired, multi-agent framework that operationalizes Conceptual Blending Theory (CBT) through a novel Schema Grammar ("G"). This structured representation decouples relational invariants from specific visual entities, providing a rigorous foundation for cross-domain logic re-instantiation. Our pipeline executes VMT through a collaborative system of specialized agents: a perception agent that distills the reference into a schema, a transfer agent that maintains generic space invariance to discover apt carriers, a generation agent for high-fidelity synthesis and a hierarchical diagnostic agent that mimics a professional critic, performing closed-loop backtracking to identify and rectify errors across abstract logic, component selection, and prompt encoding. Extensive experiments and human evaluations demonstrate that our method significantly outperforms SOTA baselines in metaphor consistency, analogy appropriateness, and visual creativity, paving the way for automated high-impact creative applications in advertising and media. Project page with source code and self-contained skills is at https://yuci-gpt.github.io/Beyond-Pixels/.

==> Figures/limitation_badcase.tex <==
\begin{figure}[!htbp]
  \centering
   % \vspace{-2em}
  \includegraphics[width=0.95\linewidth]{Images/limitation_badcase.pdf}
  % \vspace{-1.2em}
  \caption{Limitation and Badcase of our method.}
  
  \label{fig:limitation_badcase}
\end{figure}
% Our method can effectively perform garments transfer tasks with high fidelity on user intent.

==> Figures/user_study.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{Images/user_study.pdf}
  \vspace{-2.5em}
  \caption{\textbf{User study results.} }
  \label{fig:user_study}
\end{figure}
%Results generated by our method achieve the best identity alignment, editing alignment, and overall quality in user preference, showing obvious advantages compared to other methods.

==> Figures/user_study_GSB.tex <==
\begin{figure}[htbp]
  \centering
 % \vspace{-1.2em}
  \includegraphics[width=1\linewidth]{Images/user_study_GSB.pdf}
 % \vspace{-1.2em}
  \caption{GSB evaluation results.}
 % \vspace{-1em} 
  \label{fig:user_study_GSB}
\end{figure}


==> Tables/alignment.tex <==
\begin{table*}[!th]
\centering
\caption{\textbf{Comparison of similarity scores between output images and reference images, and between output images and text prompts.}.  
``Injection'' evaluates the subject identity alignment between the reference images and the output images. ``Editing'' evaluates the text alignment between the output images and the corresponding prompts.
Our method has the best scores, indicating that our approach successfully edit images guided by text while maintaining consistency with reference images and high image quality.}
% \caption{CLIP feature cosine similarity between the generated images and reference style, content and prompt. Our methods have the best average score, indicates that our approach successfully customizes the generation of the target style while preserving the content.}
\vspace{-0.5em}
\label{tab:alignment}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{DINO}$(\uparrow)$} &\multicolumn{2}{c}{\textbf{CLIP-I}$(\uparrow)$}  &\multicolumn{2}{c}{\textbf{CLIP-T}$(\uparrow)$}        &    \multirow{2}{*}{\textbf{FID$(\downarrow)$}} \\ 
\cline{2-7} &\textbf{Injection} &\textbf{Editing} &\textbf{Injection} &\textbf{Editing} &\textbf{Injection} &\textbf{Editing}             \\ \hline



Break-a-scene   	&$0.7041 \pm 0.0659$ &$\textbf{0.7087} \pm 0.0546$	&$0.7128 \pm 0.2076$ &$0.6640 \pm 0.1855$	&$0.2570 \pm 0.0230$ &$0.2820 \pm 0.0659$ &217.81\\ 
Swap-anything   	&$0.7058 \pm 0.0625$	&$0.7035 \pm 0.0556$	&$0.7275 \pm 0.1821$	&$0.7296 \pm 0.1602$	&$0.2493 \pm 0.0181$	&$0.2296 \pm 0.0354$ &190.69\\  
DreamEdit           &$0.6521 \pm 0.0625$     &$0.6477 \pm 0.0652$   &$0.7203 \pm 0.1321$   &$0.7169 \pm 0.1377$     &$0.2295 \pm 0.0562$     &$0.2271 \pm 0.0557$ &$176.21$\\ 
IC-LoRA           &$0.7005\pm 0.0631$     &$0.6855 \pm 0.0621$   &$0.6891 \pm 0.1422$   &$0.6511 \pm 0.1325$     &$0.2523 \pm 0.0367$     &$0.2624 \pm 0.0522$ &$149.75$\\ \hline
DB+Paint-by-example    &$0.7037 \pm 0.0601$    &$0.6955 \pm 0.0442$    &$0.7162 \pm 0.0193$    &$0.6841 \pm 0.0167$    &$0.2668 \pm 0.0205$      &$0.2385 \pm 0.0343$  &$172.33$\\
MimicBrush+TurboEdit &$0.7044 \pm 0.0511$ &$0.6951 \pm 0.0502$ &$0.7107 \pm 0.1337$ &$0.6991 \pm 0.1851$ &$0.2674 \pm 0.0366$ &$0.2551 \pm 0.0621$ & 153.28 \\ \hline
TF-ICON & $0.7053 \pm 0.0280$ & $0.7061 \pm 0.0225$ & $0.7235 \pm 0.1188$ & $0.7018 \pm 0.1542$ & $0.2334 \pm 0.0270$ & $0.2234 \pm 0.0297$ &169.04\\
TIGIC & $0.6901 \pm 0.0231$ & $0.6906 \pm 0.0302$ & $0.7145 \pm 0.1744$ & $0.6789 \pm 0.2012$ & $0.2656 \pm 0.0313$ & $0.2272 \pm 0.0631$ &179.07\\
PrimeComposer & $0.7029 \pm 0.0510$ & $0.6931 \pm 0.0476$ & $0.7124 \pm 0.1128$ & $0.7426 \pm 0.0619$ & $0.2609 \pm 0.0163$ & $0.2300 \pm 0.0532$ &166.85\\
Diptych & $0.6559 \pm 0.0679$ & $0.6531 \pm 0.0691$ & $0.7225 \pm 0.1287$ & $0.7145 \pm 0.1140$ & $0.2321 \pm 0.0569$ & $0.2287 \pm 0.0403$ &179.28\\ \hline
Flux-Fill & $0.6798 \pm 0.0602$ & $0.6761 \pm 0.0497$ & $0.7668 \pm 0.1274$ & $0.7843 \pm 0.1124$ & $0.2634 \pm 0.0213$ & $0.2667 \pm 0.0288$ &127.18\\ 
Ours w/o head   &$0.7115 \pm 0.0564$ &$0.6891 \pm 0.0484$ &$0.7882 \pm 0.1201$ &$0.7889 \pm 0.1121$  &$0.2621 \pm 0.186$ &$0.2682 \pm 0.331$ &$123.82$ \\ 
Ours w/o blend  &$0.7116 \pm 0.0591$ &$0.6902 \pm 0.0519$ &$0.7901 \pm 0.1192$ &$0.7869 \pm 0.1133$  &$0.2633 \pm 0.171$ &$0.2703 \pm 0.294$ &$129.47$\\ \hline
Ours & $\textbf{0.7121} \pm 0.0542$ & $0.6945 \pm 0.0563$ & $\textbf{0.7957} \pm 0.1138$ & $\textbf{0.7924} \pm 0.1113$ & $\textbf{0.2685} \pm 0.0173$ & $\textbf{0.2834} \pm 0.0365$ &\textbf{122.61}\\ \bottomrule
\vspace{-2em}
\end{tabular}
}


\end{table*}

==> Tables/alignment_ori.tex <==
\begin{table*}[!th]
\centering
\caption{\textbf{Comparison of cosine similarity between DINO features (for image) and CLIP (for text) of the edited images and target images and prompts, respectively}. Our method has the best scores, indicating that our approach successfully edit the image guided by text while maintain consistency with target image and high image quality.}
% \caption{CLIP feature cosine similarity between the generated images and reference style, content and prompt. Our methods have the best average score, indicates that our approach successfully customizes the generation of the target style while preserving the content.}
\label{tab:alignment}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c|cccccc|c}
\toprule
Methods   &TF-ICON &Break-a-scene     &Swap-anything &TIGIC &PrimeComposer &Diptych       &Ours     \\ \hline
Identity-alignment (DINO) $(\uparrow)$   	&0.8377 &0.8559	&0.8722	&0.8744		&0.8963	&0.9029 &\textbf{0.9194}\\ \hline
Prompt-alignment (CLIP) $(\uparrow)$  	&0.3019	&0.2944	&0.2975	&0.2955		&0.3022	&0.3098 &\textbf{0.3203}\\  \hline
Image-quality (LPIPS) $(\downarrow)$  &0.2151 &0.2258 &0.2975 &0.3144  &0.2796 &0.2262 &\textbf{0.2103} \\ \bottomrule
\end{tabular}
}


\end{table*}

==> Tables/user_study.tex <==



\begin{table}[t]
\centering
\caption{User Study Results. We report mean scores across 65 participants. Best results in \textbf{bold}.}
\label{tab:user_study_transposed}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Metric & BAGEL & Mid. & GPT & Banana & Ours \\
\midrule
Recogn.      & 3.66 & 3.87 & 4.06 & 4.03 & \textbf{4.34} \\
Ingenuity    & 2.94 & 3.52 & 3.63 & 3.69 & \textbf{4.57} \\
Violation    & 2.77 & 3.44 & 3.51 & 3.65 & \textbf{4.45} \\
Integration  & 4.12 & 4.18 & 4.23 & 4.49 & \textbf{4.64} \\
Visual       & 3.66 & 4.31 & 4.71 & 4.74 & \textbf{4.77} \\
\bottomrule
\end{tabular}
}
\end{table}


==> macros.tex <==
\newcommand{\tabtextsize}{\small}
\newcommand{\figtext}[1]{{\footnotesize #1}}
\newcommand{\Caption}[2]{\caption[#1]{{\footnotesize #1} {\footnotesize #2}}}

\newcommand{\invisible}[1]{{\color{white} #1}}
\newcommand{\emacsquote}[1]{{``#1''}}


\definecolor{FanColor}{rgb}{0.8,0,0.8}
\newcommand{\fan}[1]{{\color{FanColor}[Fan: #1]}}
\definecolor{YuxinColor}{rgb}{0.54,0.18,0.88}
\newcommand{\yuxin}[1]{{\color{YuxinColor}[Yuxin: #1]}}
\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\toremove}[1]{{\it\color{red} (To remove) #1}}
\newcommand{\note}[1]{{\it\color{blue} #1}}
\newcommand{\nothing}[1]{}
\newcommand{\passthrough}[1]{#1}
\newcommand{\oliver}[1]{{\color{blue}#1}}


\newcommand{\psdraftboxDefault}{\psnodraftbox}
\definecolor{figred}{rgb}{1,0,0}
\definecolor{figgreen}{rgb}{0,0.6,0}
\definecolor{figblue}{rgb}{0,0,1}
\definecolor{figpink}{rgb}{1,0.63,0.63}

\ifthenelse{\equal{\final}{1}}
{
\renewcommand{\fan}[1]{}
\renewcommand{\oliver}[1]{}
\renewcommand{\warning}[1]{}
\renewcommand{\toremove}[1]{}
\renewcommand{\note}[1]{}
}
{}

% \hyphenpenalty=1000 % magic number to reduce ugly words across two lines
% \newcommand{\bloginput}[1]{\input{blog/#1}}

\newcommand{\sectioninput}[1]{\input{Sections/#1}}

\hyphenpenalty=1000 % magic number to reduce ugly words across two lines

%\newcommand{\figureinput}[1]{\input{Figures/#1}}
\newcommand{\inputfigure}[1]{\input{Figures/#1}}
\newcommand{\tableinput}[1]{\input{Tables/#1}}

\renewcommand{\paragraph}[1]{\textbf{#1}}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}} 


==> sup/Tables/sup_alignment.tex <==
\begin{table*}[!h]
\centering
\caption{\textbf{Quantitative comparison of our method and baseline approaches \underline{across multiple random seeds}.} To evaluate the stability and consistency of the generated results, we conduct our method and all baseline methods using the same set of random seeds. The table demonstrates the consistency and robustness of our method across varying initialization conditions.}
\vspace{-0.5em}
\label{tab:sup_alignment}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{DINO}$(\uparrow)$} &\multicolumn{2}{c}{\textbf{CLIP-I}$(\uparrow)$}  &\multicolumn{2}{c}{\textbf{CLIP-T}$(\uparrow)$}        &    \multirow{2}{*}{\textbf{FID$(\downarrow)$}} \\ 
\cline{2-7} &\textbf{Injection} &\textbf{Editing} &\textbf{Injection} &\textbf{Editing} &\textbf{Injection} &\textbf{Editing}             \\ \hline
Break-a-scene  &$0.7038 \pm 0.0677$ &$\textbf{0.7088} \pm 0.0542$	&$0.7131 \pm 0.2081$ &$0.6642 \pm 0.1841$	&$0.2565 \pm 0.0239$ &$0.2822 \pm 0.0644$ &217.83\\ 
Swap-anything  &$0.7056 \pm 0.0634$	&$0.7032 \pm 0.0551$	&$0.7277 \pm 0.1816$  &$0.7291 \pm 0.1611$&$0.2494 \pm 0.0177$	&$0.2291 \pm 0.0343$ &190.72\\  \hline
DreamEdit           &$0.6524 \pm 0.0626$     &$0.6474 \pm 0.0655$   &$0.7206 \pm 0.1319$   &$0.7168 \pm 0.1375$     &$0.2297 \pm 0.0564$     &$0.2273 \pm 0.0559$ &$176.22$\\ 
IC-LoRA           &$0.7001\pm 0.0632$     &$0.6857 \pm 0.0622$   &$0.6894 \pm 0.1423$   &$0.6513 \pm 0.1327$     &$0.2518 \pm 0.0366$     &$0.2626 \pm 0.0521$ &$149.73$\\ \hline
DB+Paint-by-example    &$0.7036 \pm 0.0602$    &$0.6956 \pm 0.0441$    &$0.7161 \pm 0.0193$    &$0.6845 \pm 0.0166$    &$0.2665 \pm 0.0202$      &$0.2382 \pm 0.0341$  &$172.35$\\
MimicBrush+TurboEdit &$0.7043 \pm 0.0512$ &$0.6952 \pm 0.0504$ &$0.7105 \pm 0.1338$ &$0.6992 \pm 0.1852$ &$0.2675 \pm 0.0365$ &$0.2553 \pm 0.0624$ & 153.27 \\ \hline
TF-ICON & $0.7054 \pm 0.0275$ & $0.7064 \pm 0.0227$ & $0.7236 \pm 0.1193$ & $0.7015 \pm 0.1546$ & $0.2336 \pm 0.0265$ & $0.2237 \pm 0.0292$ &168.98\\
TIGIC & $0.6901 \pm 0.0231$ & $0.6906 \pm 0.0302$ & $0.7145 \pm 0.1744$ & $0.6789 \pm 0.2012$ & $0.2656 \pm 0.0313$ & $0.2272 \pm 0.0631$ &179.07\\
PrimeComposer & $0.7027 \pm 0.0513$ & $0.6933 \pm 0.0479$ & $0.7127 \pm 0.1133$ & $0.7424 \pm 0.0612$ & $0.2605 \pm 0.0158$ & $0.2227 \pm 0.0547$ &166.89\\
Diptych & $0.6555 \pm 0.0684$ & $0.6532 \pm 0.0685$ & $0.7228 \pm 0.1291$ & $0.7148 \pm 0.1134$ & $0.2318 \pm 0.0561$ & $0.2282 \pm 0.0412$ &179.32\\ 
Flux-Fill & $0.6801 \pm 0.0698$ & $0.6757 \pm 0.0499$ & $0.7665 \pm 0.1271$ & $0.7841 \pm 0.1127$ & $0.2637 \pm 0.0211$ & $0.2669 \pm 0.0285$ &127.16\\ \hline
Ours & $\textbf{0.7123} \pm 0.0539$ & $0.6944 \pm 0.0567$ & $\textbf{0.7959} \pm 0.1134$ & $\textbf{0.7928} \pm 0.1109$ & $\textbf{0.2689} \pm 0.0177$ & $\textbf{0.2836} \pm 0.0369$ &\textbf{122.63}\\ \bottomrule
% \textbf{Average} $(\uparrow)$    &0.4566 & 0.4623 & 0.4712  &0.4768 &0.5014   &0.5214  &\textbf{0.5383} \\ \bottomrule
\vspace{-2em}
\end{tabular}
}


\end{table*}

==> sup/supp1.tex <==
\begin{figure*}[h]
  \centering
  \includegraphics[width=0.85\linewidth]{sup/Images/supp1.pdf}
  \caption{\textbf{Additional results of our method.}}
  \label{fig:supp1}
\end{figure*}

==> sup/supp2.tex <==
\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.85\linewidth]{sup/Images/supp2.pdf}
  \caption{\textbf{Additional results of our method.}}
  \label{fig:supp2}
\end{figure*}

